The Green Monster hiding in front of Cas A: JWST reveals a dense and dusty circumstellar structure pockmarked by ejecta interactions

JWST observations of the young Galactic supernova remnant Cassiopeia A revealed an unexpected structure seen as a green emission feature in colored composite MIRI F1130W and F1280W images - hence dubbed the Green Monster - that stretches across the central parts of the remnant in projection. Combining the kinematic information from NIRSpec and MIRI MRS with the multi-wavelength imaging from NIRCam and MIRI, we associate the Green Monster with circumstellar material that was lost during an asymmetric mass-loss phase. MIRI images are dominated by dust emission but its spectra show emission lines from Ne, H and Fe with low radial velocities indicative of a CSM nature. An X-ray analysis of this feature in a companion paper (Vink et al. 2024) supports its CSM nature and detects significant blue shifting, thereby placing the Green Monster on the near side, in front of the Cas A SN remnant. The most striking features of the Green Monster are dozens of almost perfectly circular 1" - 3" sized holes, most likely created by interaction between high-velocity SN ejecta material and the CSM. Further investigation is needed to understand whether these holes were formed by small 8000-10500 km/s N-rich ejecta knots that penetrated and advanced out ahead of the remnant's 5000 - 6000 km/s outer blastwave, or by narrow ejecta fingers that protrude into the forward-shocked CSM. The detection of the Green Monster provides further evidence of the highly asymmetric mass-loss that Cas A's progenitor star underwent prior to explosion.

==> CasA_referee_report <==
Reviewer's Comments:

The paper by De Looze et al. "The Green Monster hiding in front of Cas A: . . .", thoroughly studies the `Green Monster' of Cassiopeia A core-collapse supernova remnant (CCSNR). The authors show the Green Monster is a CSM in front of the main CCSNR shell. Cassiopeia A is a key CCSNR for understanding many processes relevant to CCSNe, such as pre-explosion mass loss, the explosion mechanism, and post-explosion processes. The paper is well-written and provides detailed information for future studies and modeling. Following some minor corrections and clarifications, I recommend its publication. 

Response: We would like to thank the referee for the careful reading of the manuscript and for the very useful feedback. All suggestions have been incorporated in the new version of the paper, which are indicated in boldface in the resubmitted paper. We comment on these changes that were made to the paper below. 
 
If the authors have not done it already, I would suggest posting the paper on arXiv before final acceptance to allow the community to give comments. 

Response: We have submitted the paper to the arXiv and have explicitly requested feedback from the community. Any feedback received will be carefully considered prior to formal acceptance of the paper.

(2) Please be clear what the "ring" is. Is it the main ring of the GM? Consider pointing at it in Figure 1 and/or 2. 
Or are the rings the small rings around the small holes? You can point at the rings around the holes. If you use `ring' for both, then this is confusing. Also, maybe you can point at 2-3 holes in Figure 2 so the reader knows what you are referring to just from the figure. 

Response: We would like to thank the referee for this very useful suggestion. We have gone through the paper to make sure that the references to the specific GM ring in P2 with targeted MRS observations are clear, and can not be confused with any other GM rings. We have also highlighted the position P2 in Figure 2 to guide the eye.

(3) Line 720: "Scenario II: they result from interactions of high-velocity ejecta filaments with dense circumstellar clumps on the rear side of CasA." Do you mean "rear" or "near"? 

Response: In this specific sentence, it should be rear side. The green monster is located on the near side, but in this specific scenario, we outline a possible interpretation of the GM emission based on the partial overlap between the GM emission and a redshifted ejecta filament on the rear side of the remnant. In Section 4.2, we argue that this red-shifted high-velocity ejecta filament happens to be along the same line-of-sight where the emission of a GM ring is targeted with the JWST MIRI MRS instrument, but has no physical connection with the GM structure.

(4) The sentence: " . . postulated that small, high density fragments would have little dynamical impact on the shell, and would leave an expanding rings of compressed material." repeats itself in lines 1048 and 1052.

Response: We thank the referee for spotting this. We removed the second sentence: “Braun et al. (1987) also postulated that small, high density fragments would have little dynamical impact on the shell, and  would leave an expanding rings of compressed material. ”

(5) Last sentence of section 5: "QSFs. A similar scenario has been suggested for SN 1987A's pre-explosion stellar evolution (Morris & Podsiadlowski 2007)." 
SN 1987A has lost mass in a more or less axially-symmetric morphology, not one-sided. In planetary nebulae, highly asymmetrical mass loss with one side much denser (brighter/larger) than the other is attributed to triple-star interaction (e.g., Bear E., Soker N., 2017, ApJL, 837, L10).

Response: In this sentence, our intension was to highlight the similarity in the suggested merging scenario taking place prior to explosion in the progenitor systems of both Cas A and SN1987A. We have clarified this now in the text, and we have also added the difference in the morphology of the mass loss resulting from the stellar merging in both progenitor systems. 
We would also like to thank the referee for pointing out how asymmetric mass loss has been explained in PNe. We have added this to the text and have emphasised that the complex nature of the Cas A progenitor system will require future investigations to unravel the origin of the highly asymmetric mass loss phase that resulted in the QSFs and GM.

In addition to these requested changes, we have made minor changes to the text to enhance the readability (all changes indicated in boldface). We have also clarified in the second-to-last paragraph of Section 4.3.2 that the time gap between the ejecta bullets piercing holes in the GM and the first impact by the forward shock is around 15 to 45 years, given that the impact would have likely occurred around 45-75 years ago and given that the GM has been (partly) visible in Spitzer and ISO data, implying that the GM material has been shock heated for (at least) 30 years.


==========================
Data Editor's review:

One of our expert data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.

It is great that the authors have minted a DOI for the MAST data used in their article. The next step is to include this DOI in the revised manuscript. Ideally, the authors should use the AASTeX "\dataset" command to mark up the DOI so it can be properly tagged in production. An example would be text similar to this: 

"Some/all of the data presented in this article were obtained from the Mikulski Archive for Space Telescopes (MAST) at the Space Telescope Science Institute. The specific observations analyzed can be accessed via \dataset[doi: 10.17909/szf2-bg42]{https://doi.org/10.17909/szf2-bg42}." 
Response: We have added the info about the data and the associated doi to the acknowledgments of the paper.

